Learning Dual Transformers for All-In-One Image Restoration from a Frequency Perspective

This work aims to tackle the all-in-one image restoration task, which seeks to handle multiple types of degradation with a single model. The primary challenge is to extract degradation representations from the input degraded images and use them to guide the model's adaptation to specific degradation types. Building on the insight that various degradations affect image content differently across frequency bands, we propose a new dual-transformer approach comprising two components: a frequency-aware Degradation estimation transformer (Dformer) and a degradation-adaptive Restoration transformer (Rformer). The Dformer captures the essential characteristics of various degradations by decomposing the input into different frequency components. By understanding how degradations affect these frequency components, the Dformer learns robust priors that effectively guide the restoration process. The Rformer then employs a degradation-adaptive self-attention module to selectively focus on the most affected frequency components, guided by the learned degradation representations. Extensive experimental results demonstrate that our approach outperforms existing methods in five representative restoration tasks, including denoising, deraining, dehazing, deblurring, and low-light enhancement. Additionally, our method offers benefits for handling, real-world degradations, spatially variant degradations, and unseen degradation levels.

==> comments.tex <==


 2. The computational cost comparisons are lacking, like the number of parameters, FLOPS, inference time.

Computational complexity. The paper should include a comparison of parameters, computational complexity, and runtime of the proposed methods. It is important to show that
any performance improvements result from the novel design rather than just an increase in parameters or computation.

 3. Frequency-aware Transformer block and Degradation-adaptive restoration transformer are not described with sufficient mathematical detail, hindering understanding and potential
 implementation. The Intra-band Self-Attention mechanism is poorly explained, leaving unclear how calculations are performed among sub-band pairs. The Degradation-Aware Self-Attention module presentation is inconsistent, with the unexplained absence of the V component in Figure 1(c). 

4. The Experiment section of this manuscript lacks sufficient depth and critical analysis. A major concern is the significant performance drop in Image Dehazing (29.2 PSNR compared to PromptIR's 30.58), which is not adequately explained or analyzed.

5.The overall framework figure should be significantly improved. In the schematic diagram of the method structure shown in Figure 1, the proposed method is not clearly described; for example, there is no legend. Some parameters are unclear in meaning, such as Z1, Z2. Does the downward arrow at the top of the figure represent downsampling? The R-former only presents a basic module, and the overall architecture is not provided. Additionally, there is no relevant description found in the text of the paper.

The figures in this paper need improvement. For example, Figure 1 can not illustrate the
 framework well. Figure 1 (b) and (c) are just the special situation of 2 cases. It is difficult for us
 to distinguish the performance difference of different methods from Figure 2.






reference：

 For instance, notable studies such as "Adverse Weather Removal with Codebook
 Priors" by Tian Ye et al.
 "Learning Weather-General and Weather-Specific Features for Image
 Restoration Under Multiple Adverse Weather Conditions" by Yurui Zhu et al., and "Controlling
 Vision-Language Models for Universal Image Restoration" by Ziwei Luo et al. are not mentioned
 or discussed. 

  [1] Language-driven All-in-one Adverse Weather Removal (CVPR 2024)
 [2] Text-IF: Leveraging Semantic Text Guidance for Degradation-Aware and Interactive Image
 Fusion (CVPR 2024)
 [3] Unifying Image Processing as Visual Prompting Question Answering (ICML 2024


 [c2] Unsupervised degradation representation learning for blind super-resolution
 [c3] Learning degradation-invariant representation for robust real-world person re-identification
 [c4] LLDiffusion: Learning degradation representations in diffusion models for low-light image
 enhancement
 [c5]  Learning degradation representations for image deblurring

==> temp.tex <==
%Inter-Band Attention is the only module in the Encoder that explicitly establish interactions between different frequency bands. By strictly controlling the interactions between bands, it aims to alleviate the model's fixed frequency bias and mitigate the neglect of different frequency preferences of different degradation types. This module provides a degradation representation for each frequency band and uses a simple projection to provide per-band modulation parameters, replacing the traditional approach of using different modules for different tasks in multi-task learning, and treating all degradation types equally in an all-in-one manner. Furthermore, the scaling parameters learned by the Encoder can handle the frequency characteristics of different degradation types more finely compared to directly learnable modulation parameters, which can also be aware the spatial heterogeneity of the same degradation across different images and different regions within the same image, further mitigating the performance loss

%\textbf{Intra- \& Inter-Band Attention.}

%Recent research \cite{} has uncovered that the self-attention mechanism within Transformer-like architectures functions akin to a low-pass filter, forming the basis of frequency biases in Transformers. Consequently, it becomes feasible to modulate the filtering prowess of models by adjusting the weights of various frequency bands within attention maps, aligning with the distinct frequency demands of diverse degradation scenarios. For instance, tasks such as denoising and deraining necessitate the suppression of high-frequency noise, whereas dehazing and deblurring tasks focus on reinstating high-frequency details.

%\textit{[Note: I didn't mention Uformer since it was not designed by us, so I didn't describe how Uformer was trained or the L1 Loss and frequency domain L1 Loss either. Currently, what I have written in the methods section mainly focuses on the generality of the Encoder. I think it's better to mention that we used a Decoder based on Uformer without the learnable modulator in Experiment section, or alternatively, a Swin Transformer with the LeFF module added, which are the same.]}

%It introduces a gated mechanism in the FFN to discriminatively determine which low- and high-frequency information should be preserved for latent clear image restoration.
%Inspired by recent findings that self-attention is a low-pass filter and low-frequency signals/components are more informative to ViTs

%we propose to learn a neural degradation representation (NDR)that effectively captures the essential characteristics of various degradations. By leveraging NDR, our proposed all-in-one image restoration network, named NDR-Restore, can accurately identify and utilize the specific degradation of the input image, enabling adaptive restoration within a single network. Unlike existing representation learning methods [25], [26] that focus on capturing contents and texture details, NDR is specifically designed to learn the degradation representation. This not only allows NDR-Restore to leverage the crucial degradation information for image restoration, but also enables training NDR-Restore in an end-to-end way

%To be specific, for the Windows-based Multi-head Self Attention in the $i$-th layer of the original Swin Transformer, the number of tokens is $\frac {H_iW_i} {T^2}$, and token size is $(B, \frac {2^iC} {{nH}_i}, {nH}_i, T^2)$, where $T$ represents the length and width of the windows, and $nH \in \mathbb{R}^{M}$ denotes the number of heads in each stage. Here, $H_i=\frac{H} {2^{i}}$ and $W_i=\frac{W} {2^{i}}$, representing the length and width of the feature map in the $i$-th layer, respectively. In our proposed Encoder, we increase the size of the feature map by a factor of $L$ and incorporate the $L$ frequency dimension into the token count in both the Intra- \& Inter-Band Attention, resulting in a total of $L\times \frac {H_iW_i} {T^2}$ tokens. We apply Swin Transformer's mask mechanism to the tokens between different frequency bands and within the same frequency band in the Attention Map to achieve the desired limitation on interactions in the Intra- \& Inter-Band Attention, respectively. 


In the context of image restoration tasks, different degradation types exhibit different characteristics in terms of frequency optimization. For example, denoising and deraining tasks aim to suppress high-frequency noise, while dehazing and deblurring tasks aim to restore high-frequency details. Therefore, using the same attention map for different degradation types in all-in-one image restoration would overlook the frequency differences among various degradation types, leading to undesired performance. 
% 
However, 
Conversely, if we can flexibly adjust the filtering capability of the attention maps based on the degradation type, we can enhance the adaptability of Transformer-like models to different degradation types, effectively improving model performance. 
%

\begin{align}\label{eq-1}
    \begin{split}
        \operatorname{AMap}(\boldsymbol{X},\boldsymbol{W}_K, \boldsymbol{W}_Q)=softmax(\frac{\boldsymbol{X} \boldsymbol{W}_Q(\boldsymbol{X} \boldsymbol{W}_K)^T}{\sqrt{d}}), \\
        \operatorname{Attention}(\boldsymbol{X}\boldsymbol{W}_V)=\operatorname{AMap}(\boldsymbol{X}) \boldsymbol{X} \boldsymbol{W}_V,
    \end{split}
\end{align}


\subsection{Toy experiment for analyzing frequency learning and degradations}
To demonstrate the correlation between frequency scaling of attention maps and the frequency learning objective in image restoration, we directly apply the aforementioned frequency scaling method to a widely used image restoration framework Uformer-B. For each layer and each head, a set of learnable frequency scaling parameters $\boldsymbol{M} \in \mathbb{R}^{L-1}$ is defined, where the number of frequency bands is set to $L=2$ and $L=5$. Then, Gaussian noise with standard deviations of $\sigma=15,25,50,75$ is injected into the BSD68 dataset, and the model is trained on four denoising tasks individually. After the frequency scaling parameters reach stability, their trends are observed, as shown in the table below \textit{[Note: The current table is just a simple demo, but the data is real]}. Here, avg $\boldsymbol{M}_{k}$ denotes the average value of the learnable modulation parameters $\boldsymbol{M}_{k}$ for the $(k+1)$-th frequency band in each layer and each head of the model. In Transformers, attention maps in different layers play different roles, and the differences between different heads provide diversity. To eliminate these differences and focus only on the differences between frequency bands, a simple averaging processing is performed here.

\begin{tabular}{|c|c|c|c|c|}
  \hline
  L=2 & $\sigma=15$ & $\sigma=25$ & $\sigma=50$ & $\sigma=75$ \\
  \hline
  avg $\boldsymbol{M}_{1}$ & 16.84\% & 12.58\% & 8.10\% & 7.99\% \\
  \hline
\end{tabular}

\

\begin{tabular}{|c|c|c|c|c|}
  \hline
  L=5 & $\sigma=15$ & $\sigma=25$ & $\sigma=50$ & $\sigma=75$ \\
  \hline
  avg $\boldsymbol{M}_{1}$ & -0.07\% & -0.44\% & -0.99\% & -0.86\% \\
  \hline
  avg $\boldsymbol{M}_{2}$ & 1.75\% & 0.78\% & 0.13\% & -0.09\% \\
  \hline
  avg $\boldsymbol{M}_{3}$ & 3.47\% & 2.21\% & 1.15\% & 0.89\% \\
  \hline
  avg $\boldsymbol{M}_{4}$ & 8.96\% & 8.27\% & 7.03\% & 6.12\% \\
  \hline
\end{tabular}

From the table, we can observe that the learned frequency scaling parameters show a positive correlation with the intensity of the noise. In other words, as the noise intensity increases, there is a greater need to suppress high-frequency noise, resulting in smaller scaling parameters for high frequencies. Therefore, we can preliminarily conclude that the filtering function reflected by the learned frequency scaling parameters in image restoration is consistent with the frequency optimization objective in denoising tasks. Consequently, different scaling parameters can be used for each degradation type in the all-in-one task to modify the previously simple filtering function of the attention mechanism, better adapting to the frequency differences between different degradation types.

%To allow Tranformer-like frameworks to apply different scaling parameters to different degradation types without recognizing the degradation type in all-in-one task, we propose a frequency learning framework based on contrastive learning. It obtains a degradation representation for each frequency band separately and uses the embedded degradation representation instead of the previously learnable frequency scaling parameters. Compared to the learnable scaling parameters mentioned in the previous section, the proposed framework not only takes into account the frequency differences between different degradation types but also captures the differences between different images within the same degradation type and the differences in different spatial positions of the same image, thereby providing more detailed image restoration capabilities. In Part A, we first describe the overall process of extracting frequency contrast details for all frequency bands using the designed Encoder\textit{[Note: I didn't name any modules.]} in a discrimination-free manner. Then in Part B, we explain how the obtained degradation representation is embedded into a Transformer-based image restoration architecture using scaled attention maps.


%
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison on multiple degradations.}}
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
\multirow{2}{*}{ D-Types } & \multirow{2}{*}{ Method } & \multicolumn{3}{c}{ Denoise } & Derain & Dehaze & Deblur \\
\cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}  \cmidrule(lr){8-8} 
&& BSD68 $(\sigma=15)$ & BSD68 $(\sigma=25)$ & BSD68 $(\sigma=50)$ & Rain100L & SOTS & GOPro \\
\hline \multirow{2}{*}{ 1 } 
& AirNet & 34.14/0.9355 & 31.49/0.8928 & 28.23/0.8058 & - & - & - \\
& Ours & 34.74/0.9430 & 31.98/0.9027 & 28.66/0.8196 & - & - & - \\
\hline \multirow{2}{*}{ 2} 
& AirNet & 34.11/0.9352 & 31.46/0.8923 & 28.19/0.8042 & 38.31/0.9824 & - & - \\
& Ours & 34.69/0.9425 & 31.93/0.9020 & 28.59/0.8177 & 38.93/0.9842 & - & - \\
\hline \multirow{2}{*}{ 3} 
& AirNet & 33.92/0.9330 & 31.26/0.8881 & 28.01/0.7976 & 34.90/0.9675 & 27.94/0.9615 & - \\
& Ours & 34.59/0.9414 & 31.83/0.9000 & 28.46/0.8135 & 37.50/0.9799 & 29.20/0.9724 & - \\
\hline \multirow{2}{*}{ 4} 
& AirNet & 33.89/0.9326 & 31.21/0.8871 & 27.97/0.7950 & 34.70/0.9639 & 27.41/0.9560 & 26.36/0.7990 \\
& Ours & 34.58/0.9413 & 31.83/0.8999 & 28.46/0.8128 & 37.35/0.9795 & 28.93/0.9716 & 27.42/0.8286 \\
\bottomrule
\end{tabular}}
\label{tab:multiple}
\end{table*}
%

%
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison on various combined degradations.} in terms of two degradation types.}
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
\multirow{2}{*}{ Method } & \multicolumn{3}{c}{ Denoise } & Derain & Dehaze & Deblur \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} 
&BSD68 $(\sigma=15)$ & BSD68 $(\sigma=25)$ & BSD68 $(\sigma=50)$ & Rain100L & SOTS & GOPro \\
\hline
AirNet & 34.11/0.935 & 31.46/0.892 & 28.19/0.804 & 38.31/0.982 & - & - \\
PromptIR & 34.26/0.937 & 31.61/0.895 & 28.37/0.810 & \textbf{39.32}/\textbf{0.986} & - & - \\
Ours & \textbf{34.69}/\textbf{0.942} & \textbf{31.93}/\textbf{0.902} & \textbf{28.59}/\textbf{0.818} & \textbf{38.93}/\textbf{0.984} & - & - \\
\hline
AirNet & 33.97/0.9337 & 31.32/0.8891 & 28.06/0.7992 & - & 23.72/0.9375 & - \\
PromptIR & 33.69/0.928 & 31.03/0.880 & 27.74/0.778 & - & 30.09/0.975 & - \\
Ours & \textbf{34.66}/\textbf{0.942} & \textbf{31.91}/\textbf{0.902} & \textbf{28.56}/\textbf{0.818} & - & \textbf{29.01}/\textbf{0.972} & - \\
\hline
AirNet & 34.07/0.9346 & 31.41/0.8905 & 28.15/0.8019 & - & - & 27.90/0.8409 \\
Ours & 34.67/0.9423 & 31.92/0.9016 & 28.57/0.8170 & - & - & 29.05/0.8714 \\
\hline
AirNet & - & - & - & 32.50/0.9465 & 26.78/0.9577 & - \\
Ours & - & - & - & 36.55/0.9759 & 28.64/0.9706 & - \\
\hline
AirNet & - & - & - & 36.41/0.9548 & - & 27.43/0.8289 \\
Ours & - & - & - & 37.99/0.9813 & - & 28.69/0.8626 \\
\hline
AirNet & - & - & - & - & 20.32/0.8355 & 22.49/0.7402 \\
Ours & - & - & - & - & 28.02/0.9675 & 26.74/0.8091 \\
\bottomrule
\end{tabular}}
\label{tab:combined-2}
\end{table*}
%
%

%
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison on various combined degradations.} in terms of two degradation types.}
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
\multirow{2}{*}{ Method } & \multicolumn{3}{c}{ Denoise } & Derain & Dehaze & Deblur \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} 
&BSD68 $(\sigma=15)$ & BSD68 $(\sigma=25)$ & BSD68 $(\sigma=50)$ & Rain100L & SOTS & GOPro \\
\hline
AirNet & 34.11/0.935 & 31.46/0.892 & 28.19/0.804 & 38.31/0.982 & - & - \\
PromptIR & 34.26/0.937 & 31.61/0.895 & 28.37/0.810 & \textbf{39.32}/\textbf{0.986} & - & - \\
\textit{Ours} & \textbf{34.69}/\textbf{0.942} & \textbf{31.93}/\textbf{0.902} & \textbf{28.59}/\textbf{0.818} & 38.93/0.984 & - & - \\
\hline
%\hline
AirNet & 33.97/0.9337 & 31.32/0.8891 & 28.06/0.7992 & - & 23.72/0.9375 & - \\
PromptIR & 33.69/0.928 & 31.03/0.880 & 27.74/0.778 & - & \textbf{30.09}/\textbf{0.975} & - \\
\textit{Ours} & \textbf{34.66}/\textbf{0.942} & \textbf{31.91}/\textbf{0.902} & \textbf{28.56}/\textbf{0.818} & - & 29.01/0.972 & - \\
%\hline
%AirNet & 34.07/0.9346 & 31.41/0.8905 & 28.15/0.8019 & - & - & 27.90/0.8409 \\
%Ours & 34.67/0.9423 & 31.92/0.9016 & 28.57/0.8170 & - & - & 29.05/0.8714 \\
\hline
AirNet & - & - & - & 32.50/0.9465 & 26.78/0.9577 & - \\
PromptIR & - & - & - & 35.12/0.969 & \textbf{30.36}/\textbf{0.973} & - \\
\textit{Ours} & - & - & - & \textbf{36.55}/\textbf{0.976} & 28.64/0.9706 & - \\
%\hline
%AirNet & - & - & - & 36.41/0.9548 & - & 27.43/0.8289 \\
%Ours & - & - & - & 37.99/0.9813 & - & 28.69/0.8626 \\
%\hline
%AirNet & - & - & - & - & 20.32/0.8355 & 22.49/0.7402 \\
%Ours & - & - & - & - & 28.02/0.9675 & 26.74/0.8091 \\
\bottomrule
\end{tabular}}
\label{tab:combined-2}
\end{table*}
%




%
\begin{table*}[t!]
\centering
\caption{\textbf{Comparison on various combined degradations} in terms of three degradation types.}
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
\multirow{2}{*}{ Method } & \multicolumn{3}{c}{ Denoise } & Derain & Dehaze & Deblur \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7} 
& BSD68 $(\sigma=15)$ & BSD68 $(\sigma=25)$ & BSD68 $(\sigma=50)$ & Rain100L & SOTS & GOPro \\
\hline 
AirNet & 33.92/0.9330 & 31.26/0.8881 & 28.01/0.7976 & 34.90/0.9675 & 27.94/0.9615 & - \\
Ours & 34.59/0.9414 & 31.83/0.9000 & 28.46/0.8135 & 37.50/0.9799 & 29.20/0.9724 & - \\
\hline 
AirNet & 34.05/0.9343 & 31.37/0.8899 & 28.14/0.8003 & 37.50/0.9787 & - & 28.01/0.8451 \\
Ours & 34.65/0.9421 & 31.89/0.9013 & 28.54/0.8159 & 38.72/0.9835 & - & 28.99/0.8699 \\
\hline 
AirNet & 33.92/0.9329 & 31.26/0.8881 & 28.03/0.7976 & - & 27.17/0.9548 & 26.40/0.8013 \\
Ours & 34.62/0.9419 & 31.87/0.9007 & 28.52/0.8151 & - & 28.65/0.9695 & 28.23/0.8511 \\
\hline 
AirNet & - & - & - & 32.76/0.9474 & 25.67/0.9419 & 25.96/0.7887 \\
Ours & - & - & - & 36.03/0.9738 & 28.15/0.9678 & 26.70/0.8092 \\
\bottomrule
\end{tabular}}
\label{tab:combined-3}
\end{table*}

%%
\begin{table*}[t!]
\centering
\caption{\textbf{Ablation staudy.} "w.o. intra-inter" means replacing the dual MSA with the regular MSA;"w.o. Contrast" means removing the entire contrastive learning encoder;"w.o. Decompose" means removing the initial frequency decomposition in the encoder and replacing the dual MSA with the regular MSA..}
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
\multirow{2}{*}{ D-Types } & \multirow{2}{*}{ Method } & \multicolumn{3}{c}{ Denoise } & Derain & Dehaze & Deblur \\
\cmidrule(lr){3-5} \cmidrule(lr){6-6} \cmidrule(lr){7-7}  \cmidrule(lr){8-8} 
& & BSD68 $(\sigma=15)$ & BSD68 $(\sigma=25)$ & BSD68 $(\sigma=50)$ & Rain100L & SOTS & GOPro \\
\hline \multirow{4}{*}{ 3 } 
& w.o. intra-inter & 34.59/0.9413 & 31.83/0.8997 & 28.48/0.8134 & 37.45/0.9798 & 28.72/0.9707 & - \\
& w.o. Contrast & 34.59/0.9417 & 31.84/0.9002 & 28.48/0.8135 & 37.42/0.9801 & 28.17/0.9684 & - \\
& w.o. Decompose & 34.44/0.9397 & 31.71/0.8975 & 28.35/0.8089 & 35.50/0.9700 & 28.38/0.9683 & - \\
& Ours & 34.59/0.9414 & 31.83/0.9000 & 28.46/0.8135 & 37.50/0.9799 & 29.20/0.9724 & - \\
\hline \multirow{3}{*}{ 4(Abandoned) } 
& w.o. intra-inter & 34.57/0.9413 & 31.81/0.8996 & 28.44/0.8120 & 37.37/0.9794 & 28.67/0.9695 & 27.41/0.8290 \\
& w.o. Contrast & 34.59/0.9416 & 31.83/0.9003 & 28.47/0.8130 & 37.35/0.9795 & 28.34/0.9682 & 27.56/0.8317 \\
& Ours & 34.58/0.9413 & 31.83/0.8999 & 28.46/0.8128 & 37.35/0.9795 & 28.93/0.9716 & 27.42/0.8286\\
\bottomrule
\end{tabular}}
\label{tab:ablation}
\end{table*}

%Firstly, the self-attention matrixs in the restoration transformer are decomposed into low-frequency and high-frequency components. Subsequently, the ratio between these components is dynamically adjusted with the guidance of the acquired degradation prior.
